A Hardware-Software Blueprint for Flexible Deep Learning Specialization

Specialized Deep Learning (DL) acceleration stacks, designed for a specific set of frameworks, model architectures, operators, and data types, offer the allure of high performance while sacrificing flexibility. Changes in algorithms, models, operators, or numerical systems threaten the viability of specialized hardware accelerators. We propose VTA, a programmable deep learning architecture template designed to be extensible in the face of evolving workloads. VTA achieves this flexibility via a parametrizable architecture, two-level ISA, and a JIT compiler. The two-level ISA is based on (1) a task-ISA that explicitly orchestrates concurrent compute and memory tasks and (2) a microcode-ISA which implements a wide variety of operators with single-cycle tensor-tensor operations. Next, we propose a runtime system equipped with a JIT compiler for flexible code-generation and heterogeneous execution that enables effective use of the VTA architecture. VTA is integrated and open-sourced into Apache TVM, a state-of-the-art deep learning compilation stack that provides flexibility for diverse models and divergent hardware backends. We propose a flow that performs design space exploration to generate a customized hardware architecture and software operator library that can be leveraged by mainstream learning frameworks. We demonstrate our approach by deploying optimized deep learning models used for object classification and style transfer on edge-class FPGAs.

==> 06-related.tex <==
\section{Related Work}

\paragraph{Deep Learning Accelerators}
There has been an explosion of deep learning accelerator design proposals from academia~\cite{Chen:DaDianNao, Chen:Eyeriss, Han:EIE, Liu:PuDianNao, Du:ShiDianNao} and industry~\cite{Jouppi:TPU,chung2018serving,deephi,nvdla,Liu:Cambricon}. Rather than focusing solely on hardware design, \accel proposes a new two-level ISA with a simple hardware architecture and provides a complete blueprint for building a custom deep learning accelerator stack. Our work provides a co-designed runtime and hardware design which leverages off-the-shelf graph and operator compilers to facilitate the generation of optimized deep learning libraries for diverse workloads.

\paragraph{Model-to-FPGA Compilers}
Model to FPGA translation is an active area of research~\cite{sharma:dnnweaver,Umuroglu:FINN,chung2018serving,blott2018finn,abdelfattah2018dla}.
DNNWeaver~\cite{sharma:dnnweaver} implements a compiler from Caffe to static templatized FPGA accelerator, guided by a heuristic algorithm that aims to minimize off-chip memory accesses. Our approach differs from that of the DNNWeaver optimization framework, because we offload graph/schedule optimization to existing optimization toolchains (Relay~\cite{roesch2018relay}, TVM~\cite{Chen:TVM}), and design a runtime that exposes
necessary knobs to offload graph and schedule optimizations to the upper layers of the stack, allowing for end-to-end tuning. To the best of our knowledge, model-to-FPGA compilers do not cover graph and operator optimization tools~\cite{Chen:TVM,Wei:DLVM,Vasilache:TensorComprehensions,fbglow}. Most importantly, though, our work on \accel is not about spatially porting models to FPGAs but about a principled two-level ISA design and low-complexity micro-architecture, which is applicable to both FGPA-based deployment as well as custom silicon. 

BrainWave~\cite{chung2018serving} is a cloud-scale DNN acceleration framework that relies on a spatially distributed microarchitecture that can scale across many \mbox{FPGAs} while keeping neural network parameters on chip, reducing data movement from DRAM. \accel, on the other hand, targets edge class FPGAs that have limited storage (< 1MB). For that reason, we are reliant upon tiling, and latency hiding strategies to maximize compute resource utilization.

\paragraph{Narrow Precision and Model Compression}
There has been extensive work on maximizing hardware inference efficiency using binarization~\cite{Umuroglu:FINN}, and weight and activation quantization~\cite{judd2016stripes, reagen2016minerva}.
Much of the complexity involved in supporting hardware inference lies in improving training techniques~\cite{rastegari2016xnor,Courbariaux:BinaryConnect,zhou2016dorefa,cai2017deep}, and adapting a deep learning framework to support new data layouts imposed by quantized data types. In \accel's evaluation, we tackle the challenges of training quantized networks by modifying a complete deep learning stack to support end-to-end inference.

Model compression is a popular technique that prunes model parameters~\cite{Han:DeepCompression,Han:EIE,Albericio:Cnvlutin,reagen2016minerva} with minimal accuracy loss to reduce data movement and inference energy.
\accel only supports dense operators, but could be extended to support popular sparse matrix representations to take advantage of these compression techniques.




